Domain-Generalized Textured Surface Anomaly Detection

Anomaly detection aims to identify abnormal data that deviates from the normal ones, while typically requiring a sufficient amount of normal data to train the model for performing this task. Despite the success of recent anomaly detection methods, performing anomaly detection in an unseen domain remain a challenging task. In this paper, we address the task of domain-generalized textured surface anomaly detection. By observing normal and abnormal surface data across multiple source domains, our model is expected to be generalized to an unseen textured surface of interest, in which only a small number of normal data can be observed during testing. Although with only image-level labels observed in the training data, our patch-based meta-learning model exhibits promising generalization ability: not only can it generalize to unseen image domains, but it can also localize abnormal regions in the query image. Our experiments verify that our model performs favorably against state-of-the-art anomaly detection and domain generalization approaches in various settings.

==> alg_test.tex <==
\begin{algorithm}[t]
\caption{Testing stage of our method}
\label{testing}
\begin{algorithmic}
\State \textbf{Input:} $(I_Q, I_R)$ sampled from $D_{M+1}$
%; the trained feature extractor $\phi$, meta-comparer $\theta_C$, and co-attention module $\theta_A$.
\State \textbf{Output:} Image-level anomaly score $\hat{y}$ and pixel level anomaly scores $\hat{y}(p)$'s for the query image $I_Q$.
\State Extract $\phi(I_Q)$, $\phi(I_R)$ with $L$ scales
\For{$i$ in $L$}  \Comment{multi-scale features}
    \For{$j$ in $N_Q$}  \Comment{patches at scale $i$}
        \State Calculate anomaly score $s^j_i$ using eq.~\eqref{eq:s_i}
    \EndFor
\EndFor
\State Make image-level prediction $\hat{y}(I_Q)$ using eq.~\eqref{eq:im_pred}
\For{each pixel $p$ in $I_Q$} 
    \State Make pixel-level prediction $\hat{y}(p)$ using eq.~\eqref{eq:patch_pred}
\EndFor
\end{algorithmic}
\end{algorithm}

==> alg_train.tex <==
\begin{algorithm}[t]
% \algrenewcommand\textproc{}
\caption{Training stage of our method}
\label{training}
\begin{algorithmic}
% \State \textbf{Pre-Training of VAE-GAN}
\State \textbf{Input:} Source domain data $D = [D_1, ..., D_M]$
\State \textbf{Output:} The trained feature extractor $\phi$, meta-comparer $\theta_C$, and co-attention module $\theta_A$.
% \State Initialize $\phi$ with ImageNet pre-trained weights 
% \State Initialize $\theta_C$, $\theta_A$ with random parameters
\For{each iteration}
    \For{$D_m$ in $D$} \Comment{multiple source domains}
        \State Initialize $L_{cls} = L_{att} = L_{rank} = 0$
        \State Sample $I_Q$, $I_R$ from $D_m$
        \State Extract $\phi(I_Q)$, $\phi(I_R)$ with $L$ scales
        \For{$i$ in $L$}  \Comment{multi-scale features}
            \State Sample $Q_i$ from $\phi_i(I_Q)$
            \State Sample $R_i$ from $\phi_i(I_R)$
            \State $L_{cls} \gets L_{cls} +$ loss from eq.~\eqref{eq:l_cls}
            \State $L_{att} \gets L_{att} +$ loss from eq.~\eqref{eq:l_att} 
            \State $L_{rank} \gets L_{rank} +$ loss from eq.~\eqref{eq:l_rank} 
        \EndFor
        \State Update $\phi$ using $L_{cls}+L_{att}+L_{rank}$
        \State Update $\theta_C$ using $L_{cls}+L_{rank}$
        \State Update $\theta_A$ using $L_{att}+L_{rank}$
    \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}

==> backup_related.tex <==
\section{Related Works}

\noindent\textbf{Anomaly Detection} Autoencoder has been a popular model widely applied for anomaly detection. By training the autoencoder using normal training data, the model is expected to reconstruct inputs with the same data distribution; on the other hand, if an abnormal data instance is observed, the trained autoencoder would not be able to achieve satisfactory data recovery~\cite{zong2018deep}. However, it is possible to encounter the over-generalized problem; that is, it is likely to train an autoenoder which recovers abnormal data well, or the reconstruction loss might not be sufficient to reflect the data normality. To alleviate such problems, \cite{gong2019memorizing, tan2021trustmae} propose to learn memory banks to regularize the autoencoder, ensuring the data to be described by representative patterns, and promising performances have been reported. \textcolor{green}{On the other hand, \cite{schlegl2017unsupervised, akcay2018ganomaly, schlegl2019f} choose to utilize generative models which better model the distribution of normal data.} However, the learning of the above models rely on normal training data during training. Thus, the learned model cannot be directly applied to a different and unseen data domain for performing anomaly detection.\\
% \textbf{[SO WHAT ARE THE CONCERNS OR LIMITATIONS OF SUCH METHODS?]}\\

\noindent\textbf{Domain Generalization} Learning models from a single or multiple source domains, domain generalization aims to leverage this model to unseen target domains for solving the same learning task. A straightforward yet naive baseline approach for domain generalization is to aggregate training samples from all source domains to learn a single model. 
To further improve the generalization capability,
\textcolor{green}{\cite{li2018domain, yue2019domain} utilize generative adversarial network (GAN) models to generate training data with different styles, with the hope to augment diverse yet practical data distributions for training their models.}
% \textbf{more diversity (WHAT DOES THIS MEAN?)}.
\cite{li2019episodic} designs an episodic learning procedure that simulates the domain shift observed during training for deriving a domain generalized model. \cite{wang2020eis} argues that a properly learned domain generalization model would discover the image intrinsic properties, which are irrelevant to the data domains observed. Thus, self-supervised auxiliary learning tasks are introduced to prompt the learning of their models.

% \textbf{\cite{li2019feature} extends the domain generalization problem to a more challenging setting, i.e., heterogeneous domain generalization (HDG), where the unseen domains do not share label space with the seen ones. The goal of HDG is to learn a general feature representation that can apply to novel categories. The trained feature extractor is fixed after the feature learning stage, and then a split of target samples is available for training a shallow SVM or KNN classifier. (WHY MENTIONS HDG WHICH SEEMS IRRELEVANT...}

% \textbf{[WHAT ARE THE LIMITATIONS]}.
Although the recent success of domain generalization has benefited a wide range of computer vision applications, as we pointed out earlier in Section~1, it would not be possible to perform anomaly detection in unseen target domains, if no reference/normal data are observed during testing. Thus, while we tackle the task of domain-generalized anomaly detection, we consider the scenario that normal and abnormal image data are available across different source domains during training, and we expect the learned model can be applied to unseen target domains in which only a single or a number of normal images are available as the references during testing. In the following section, we will detail the setting and the design of our proposed model, and we will explain how it is able to identify defect regions with only image-level labels are observed during training.
% We summarize and compare the settings of the aforementioned learning schemes in Table~\ref{setting}.

% \textbf{[No need to repeat the technical contributions. We just did so at the end of Sect. 1]. To address the domain generalization problem for anomaly detection, we propose a model that learns how to compare patch features from the multiple source domains. With the designed image-level and patch-level objectives, our model is able to apply to an unseen target domain for both anomaly detection and localization.}

% \input{table/setting}
% \input{table/setting}

==> figure/co-attention.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=0.8\linewidth]{image/co-attention_v2.png}
\end{center}
\vspace{-0.2cm}
\caption{
Illustration of our co-attention module, which applies a linear layer to map a pair of query-reference patch features (e.g., $q^j_i$ and $r^k_i$) into a shared latent space, with the associate attention score calculated by the cosine similarity.}
\label{coatt}
\end{figure}

==> figure/meta-comparer.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=0.8\linewidth]{image/meta-comparer_v2.png}
\end{center}
\vspace{-0.2cm}
\caption{
Illustration of our meta-comparer, which learns to output the anomaly score for different query patches (i.e., $q_i^j$) in a query-reference image pair at image scale $i$.}
\label{comparer}
\end{figure}

==> figure/qps.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=\linewidth]{image/qps.png}
\end{center}
\caption{
Illustration of our feature selection strategy for the query patches. We select the patches with higher anomaly scores from the coarser scale level to reduce the computational complexity for the finer scale level.}
\label{qps}
\end{figure}

==> table/ad_dg_cross.tex <==
\begin{table*}[t]
% \scriptsize
% \footnotesize
\small
\centering

\begin{tabular}{cc|ccc|cccc}
\hline
Source         & Target     & AGG   & Epi-FCR & EISNet         & AGG+  & Epi-FCR+ & EISNet+ & Ours           \\ \hline
G, L, T, W     & Carpet     & 0.875 & 0.916   & \textbf{0.991} & 0.891 & 0.916    & 0.982   & 0.943          \\
C, L, T, W     & Grid       & 0.628 & 0.640   & 0.662          & 0.608 & 0.725    & 0.728   & \textbf{0.730} \\
C, G, T, W     & Leather    & 0.981 & 0.995   & 1.000          & 0.992 & 1.000    & 1.000   & 1.000          \\
C, G, L, W     & Tile       & 0.886 & 0.947   & 0.850          & 0.912 & 0.951    & 0.858   & \textbf{0.956} \\
C, G, L, T     & Wood       & 0.852 & 0.909   & \textbf{0.986} & 0.865 & 0.941    & 0.979   & 0.962          \\ \hline
\multicolumn{2}{c|}{Average} & 0.845 & 0.881   & 0.898          & 0.854 & 0.907    & 0.909   & \textbf{0.918} \\ \hline
\end{tabular}

\caption{Domain-generalized anomaly detection on MVTev-AD with the leave-one-domain-out setting in terms of the average image-level AUC. Note that the $+$ notation denotes the modified versions for existing DG approaches (i.e., with learn-to-compare scheme introduced).}
\label{ad_dg}
\end{table*}

==> table/ad_implement.tex <==
\begin{table}
\footnotesize
% \small
\centering


\begin{tabular}{l|ccc}
\hline
                           & AE~\cite{bergmann2018improving}     & MemAE~\cite{gong2019memorizing}  & TrustMAE~\cite{tan2021trustmae} \\ \hline
Detection (Reported)       & -      & 0.890 & 0.977   \\
Detection (Implemented)    & -      & 0.895 & 0.964   \\ \hline
Localization (Reported)    & 0.671 & 0.852 & 0.938   \\
Localization (Implemented) & 0.670 & 0.851 & 0.919     \\ \hline
\end{tabular}


\caption{Caption}
\label{ad_implement}
\end{table}

==> table/btad.tex <==
\begin{table}
\footnotesize
% \small
\centering

\begin{tabular}{ c | c  c  c | c}
	\hline
	            &   Product 1  &   Product 2    &   Product 3    &   Average \\
	\hline
	AGG~\cite{li2019episodic}    &   0.711   &   0.670   &   0.757   &   0.713   \\
    Epi-FRC~\cite{li2019episodic} &   0.841   &   0.797   &   0.725   &   0.788     \\
	EISNet~\cite{wang2020eis} &   0.917   &   0.817   &   0.916   &   0.883   \\
	\hline
    Ours   &   \textbf{0.923}   &   \textbf{0.836}   &  \textbf{0.962}   &   \textbf{0.907}\\
	\hline
\end{tabular}

\caption{Domain-generalized anomaly detection on BTAD by a model trained on MVTec-AD in terms of the average image-level AUC. Note that the $+$ notation denotes the modified versions for existing DG approaches (i.e., with learn-to-compare scheme introduced)}
\label{btad}
\end{table}

==> table/btad_cross.tex <==
\begin{table*}[t]
\small
\centering

\begin{tabular}{cc|ccc|cccc}
\hline
Source         & Target     & AGG   & Epi-FCR & EISNet         & AGG+  & Epi-FCR+ & EISNet+ & Ours           \\ \hline
MVTec     & BTAD-1    & 0.663 & 0.798   & \textbf{0.937}         & 0.711 & 0.841    & 0.917   & 0.923          \\
MVTec     & BTAD-2    & 0.634 & 0.736   & 0.812          & 0.670 & 0.797    & 0.817   & \textbf{0.836}  \\
MVTec     & BTAD-3    & 0.682 & 0.731   & 0.861          & 0.757 & 0.725    & 0.916   & \textbf{0.962}          \\ \hline
\multicolumn{2}{c|}{Average} & 0.660 & 0.755   & 0.870       & 0.713 & 0.788    & 0.883   & \textbf{0.907}   \\ \hline
\end{tabular}

\caption{Domain-generalized anomaly detection on BTAD by a model trained on MVTec-AD in terms of the average image-level AUC. Note that the $+$ notation denotes the modified versions for existing DG approaches (i.e., with learn-to-compare scheme introduced)}
\label{btad}
\end{table*}

==> table/setting.tex <==
\begin{table}
\centering
% \footnotesize
\small

\begin{tabular}{|c|c|c|}
\hline
Tasks                                                                                 & Source Data & Target Data                                                    \\ \hline\hline
Anomaly Detection                                                                     &             & Normal                                                         \\ \hline
Domain Generalization                                                                 & V           &                                                                \\ \hline
% \begin{tabular}[c]{@{}c@{}}Cross-Domain\\ Few-Shot\end{tabular}                       & V           & Few                                                            \\ \hline
% \begin{tabular}[c]{@{}c@{}}Heterogeneous\\ Domain Generalization\end{tabular}         & V           & \begin{tabular}[c]{@{}c@{}}Few /\\ No fine-tune\end{tabular}    \\ \hline
\begin{tabular}[c]{@{}c@{}}Domain Generalization for\\ Anomaly Detection\end{tabular} & V           & \begin{tabular}[c]{@{}c@{}}Normal /\\ No fine-tune\end{tabular} \\ \hline
\end{tabular}


\caption{Caption}
\label{setting}
\end{table}
